Geometry of Interest (GOI): Spatio-Temporal Destination Extraction and Partitioning in GPS Trajectory Data

Nowadays large amounts of GPS trajectory data is being continuously collected by GPS-enabled devices such as vehicles navigation systems and mobile phones. GPS trajectory data is useful for applications such as traffic management, location forecasting, and itinerary planning. Such applications often need to extract the time-stamped Sequence of Visited Locations (SVLs) of the mobile objects. The nearest neighbor query (NNQ) is the most applied method for labeling the visited locations based on the IDs of the POIs in the process of SVL generation. NNQ in some scenarios is not accurate enough. To improve the quality of the extracted SVLs, instead of using NNQ, we label the visited locations as the IDs of the POIs which geometrically intersect with the GPS observations. Intersection operator requires the accurate geometry of the points of interest which we refer to them as the Geometries of Interest (GOIs). In some application domains (e.g. movement trajectories of animals), adequate information about the POIs and their GOIs may not be available a priori, or they may not be publicly accessible and, therefore, they need to be derived from GPS trajectory data. In this paper we propose a novel method for estimating the POIs and their GOIs, which consists of three phases: (i) extracting the geometries of the stay regions; (ii) constructing the geometry of destination regions based on the extracted stay regions; and (iii) constructing the GOIs based on the geometries of the destination regions. Using the geometric similarity to known GOIs as the major evaluation criterion, the experiments we performed using long-term GPS trajectory data show that our method outperforms the existing approaches.

==> Revised GOI Journal Article/Temp.tex <==
The real SVL for the depicted scenario is $null \rightarrow d1 \rightarrow null \rightarrow d2 \rightarrow unknown \rightarrow d3 \rightarrow null$. In the generated SVL, the term null means that the GPS point can not be labeled by any of the POIs since it does not intersect with any of them. The term unknown means that, the GPS point intersects with more than one POI. Hence, the process is not able to determine a label for the observation.

==> Temp.tex <==
The real SVL for the depicted scenario is $null \rightarrow d1 \rightarrow null \rightarrow d2 \rightarrow unknown \rightarrow d3 \rightarrow null$. In the generated SVL, the term null means that the GPS point can not be labeled by any of the POIs since it does not intersect with any of them. The term unknown means that, the GPS point intersects with more than one POI. Hence, the process is not able to determine a label for the observation.
